ProbTS: Benchmarking Point and Distributional Forecasting across Diverse Prediction Horizons

Delivering precise point and distributional forecasts across a spectrum of prediction horizons represents a significant and enduring challenge in the application of time-series forecasting within various industries. Prior research on developing deep learning models for time-series forecasting has often concentrated on isolated aspects, such as long-term point forecasting or short-term probabilistic estimations. This narrow focus may result in skewed methodological choices and hinder the adaptability of these models to uncharted scenarios. While there is a rising trend in developing universal forecasting models, a thorough understanding of their advantages and drawbacks, especially regarding essential forecasting needs like point and distributional forecasts across short and long horizons, is still lacking. In this paper, we present ProbTS, a benchmark tool designed as a unified platform to evaluate these fundamental forecasting needs and to conduct a rigorous comparative analysis of numerous cutting-edge studies from recent years. We dissect the distinctive data characteristics arising from disparate forecasting requirements and elucidate how these characteristics can skew methodological preferences in typical research trajectories, which often fail to fully accommodate essential forecasting needs. Building on this, we examine the latest models for universal time-series forecasting and discover that our analyses of methodological strengths and weaknesses are also applicable to these universal models. Finally, we outline the limitations inherent in current research and underscore several avenues for future exploration.

==> analyses.tex <==
% below are prompts for GPT-4

\section{Analyses}
\label{sec:analysis}

Using \probts, we benchmark selected methods in both short-term and long-term forecasting scenarios, evaluated using both point and distributional forecast metrics.
To ensure the validity of the results and remove randomness, we run each experiment, corresponding to a dataset, a forecasting horizon, and a model, with five independent runs with different seeds for parameter initialization.
Table~\ref{tab:short_term_fore} and Table~\ref{tab:long_term_fore} shows the results for short-term and long-term, respectively,
Note that for long-term forecasting scenarios, due to too many combinations of datasets and forecasting horizons, we display the results of some further selected methods from each reserach branch, assured to incorporate the best performing one in each case.

\paragraph{Conflicts in Point and Distributional Forecast Metrics.}
Before proceeding to the analyses in terms of different methodological choices, we have widely observed optimal performance in distributional metrics does not necessarily translate to optimal performance in point forecasts.
Typical examples include  xxx in Table xx, and xxx in Table x (Leave a blank to be added later)
These observations remind us that we should compare these methods from different angles, using both NMAE and CRPS.
It is noteworthy that for point forecasting methods, these two metrics are actually equivalent.

\subsection{Analyzing customized neural architectures tailored for long-term point forecasting}

First, we have confirmed advancements in this line of research.
For example, from Table~\ref{tab:long_term_fore}, we can observe that the state-of-the-art architecture, PatchTST, is the most competitive model in most cases, especially when considering the NMAE metric.

\paragraph{However, the huge advantages of PatchTST significantly diminish in short-term forecasting scenarios.}
Our quantified data characteristics, especially non-Gaussianity, can provide proper explanations here.
Figure plots xxx (Jiawen's figure)
These analyses show that these advantages diminish may due to lacking a crucial capability: tackle complex data distribution.

\paragraph{Unfortunately, the integration of these architectures with advanced distribution estimation capabilities remains an open issue.} As will be discussed next, non-autoregressive probabilistic methods run into severe efficiency issues in long-term forecasting. Coincidentally, all these arhicetures choose non-autoreg decoding scheme. We will analyze the pros and cons between autoreg and non-autoreg in Section xx.

\subsection{Analyzing probabilistic forecasting methods developed under short-term forecasting scenarios}

At first, we also affirm the effectiveness of these probabilistic methods in their developed data scenarios.
Table~\ref{tab:short_term_fore} justifies that some pioneering methods, such as CSDI, TimeGrad, produce the most competitive results in most cases.

\paragraph{However, in long-term forecasting scenarios, those customized neural architectures, with only point forecasting objectives, can largely outperform these probabilistic methods when using distributional metrics, such as CRPS.}
Table~\ref{tab:long_term_fore} includes all these observations. Specifically, Figure xxx visualize these comparisons specifically, clearly show the gap. (@jiawen, add here)
Non-Gaussianity can provide some explanations also, because in long-term forecasting scenarios, the calcualted values are much smaller than those in short-term cases.

\paragraph{As we dive deeper, we find that these probabilistic forecasting methods have a much balanced preference for autoregressive and non-autoregressive decoding schemes, very different from those customized architectures only choosing non-autoregressive.}
For example, TimeGrad choose auto-regressive decoding, CSDI uses non-autoregressive decoding. More other examples can be found in Appendix Table~\ref{tab:categories1}.
Actually, these two decoding schemes suffer from different challenges when meeting long-term probabilistic forecasting.

\paragraph{Autoregressive probabilistiic methods, such as TimeGrad, tend to propagate more errors as the forecasting horizon or the trend strength increases.}
Figure xxx depict xxx, we observe that the performance gap increases with xxx (@Jiawen, add here)

\paragraph{Non-autoregressive probabilistic methods, such as CSDI, run into severe efficiency problems, in terms of both memory and time, in long-term forecasting scenarios.}
We have visualized this in the appendix xxx (@Jiawen, add here)

\paragraph{Interestingly, an extraordinary advantage of autoregressive decoding scheme lies in handling strong seasonality.}
Typical examples include the results for the Traffic dataset in Table~\ref{tab:long_term_fore}, where both GRU NVP and TimeGrad achieve  better results than PatchTST. It is noteworthy that GRU NVP and TimeGrad actually employ very common neural architectures.
In Figure xxx, we further investigate this finding by connecting seasonality strength with the variations of the performance gaps. (@Jiawen, add here).
We can observe a clear pattern that as the seasonality strength increases, autoregressive methods distinctly demonstrate remarkable performance.
This observation implies that autoregressive decoding scheme should not be discarded in long-term forecasting, its special binding with seasonality, probably due to more parameter-efficient, make it return to the center stage, if we find proper ways to alleviate error propagations.


Given the above logics, which is a little bit messy and not so formal, please help me to re-write to make it more structured, with good English expressions, and please try to make it concise. Please color those xxx and @Jiawen comments with red and leave it unchanged. I need her assistance to add some contents.
